Accelerated Recovery with RIS: Designing Wireless Resilience in Mission-Critical Environments

As 6G and beyond redefine connectivity, wireless networks become the foundation of critical operations, making resilience more essential than ever. With this shift, wireless systems cannot only take on vital services previously handled by wired infrastructures but also enable novel innovative applications that would not be possible with wired systems. As a result, there is a pressing demand for strategies that can adapt to dynamic channel conditions, interference, and unforeseen disruptions, ensuring seamless and reliable performance in an increasingly complex environment. Despite considerable research, existing resilience assessments lack comprehensive key performance indicators (KPIs), especially those quantifying its adaptability, which are vital for identifying a system's capacity to rapidly adapt and reallocate resources. In this work, we bridge this gap by proposing a novel framework that explicitly quantifies the adaption performance by augmenting the gradient of the system's rate function. To further enhance the network resilience, we integrate Reconfigurable Intelligent Surfaces (RISs) into our framework due to their capability to dynamically reshape the propagation environment while providing alternative channel paths. Numerical results show that gradient augmentation enhances resilience by improving adaptability under adverse conditions while proactively preparing for future disruptions.

==> figures/commands.tex <==
\newcommand{\blank}[1]{\hfil\penalty1000\hfilneg\rule[-3pt]{#1}{0.4pt}} % nice blank underscores
\newcommand{\modernBS}{
	\begin{tikzpicture}[scale=.6]
	{
		\draw (0,1) -- (0,-0.8) node [pos=0.3]  (middletop){};
		\draw (0,1) -- (0,-0.8) node [pos=0.75] (middlebot){};
		\draw (0,1) -- (0.5,-0.5) node [pos=0.3] (righttop){};
		\draw (0,1) -- (0.5,-0.5) node [pos=0.75](rightbot){};
		\draw (0,1) -- (-0.5,-0.5)node [pos=0.3] (lefttop){};
		\draw (0,1) -- (-0.5,-0.5)node [pos=0.75](leftbot){};
		\draw (-0.5,-0.5) -- (0,-0.8) -- (0.5,-0.5);
		\draw (righttop.center)-- (middletop.center) -- (lefttop.center);
		\draw (rightbot.center)-- (middlebot.center) -- (leftbot.center);
	}
	\end{tikzpicture}	
}

\newcommand{\modernBSHalo}{
	\begin{tikzpicture}[scale=.6]
	{
		\draw (0,1) -- (0,-0.8) node [pos=0.3]  (middletop){};
		\draw (0,1) -- (0,-0.8) node [pos=0.75] (middlebot){};
		\draw (0,1) -- (0.5,-0.5) node [pos=0.3] (righttop){};
		\draw (0,1) -- (0.5,-0.5) node [pos=0.75](rightbot){};
		\draw (0,1) -- (-0.5,-0.5)node [pos=0.3] (lefttop){};
		\draw (0,1) -- (-0.5,-0.5)node [pos=0.75](leftbot){};
		\draw (-0.5,-0.5) -- (0,-0.8) -- (0.5,-0.5);
		\draw (righttop.center)-- (middletop.center) -- (lefttop.center);
		\draw (rightbot.center)-- (middlebot.center) -- (leftbot.center);

      \draw[yshift=1cm] (0,0.1) ++(-10:.1) arc (10:180-10:.1);
      \draw[yshift=1cm] (0,0.2) ++(-10:.3) arc (10:180-10:.3);
	}
	\end{tikzpicture}	
}

\newcommand{\modernBuildingWindow}{
   \begin{tikzpicture}
%      \node[rectangle,draw,minimum width=] at (0,0){};
   \end{tikzpicture}
}

\newcommand{\modernBuilding}{
	\begin{tikzpicture}[scale=2]
	{
		\draw (0,1) -- (0,-0.8) node [pos=0.9]  (middletop){};
		\draw (0.5,1.3) -- (0.5,-0.5) node [pos=0.9] (righttop){};
      \draw (-0.5,1.3) -- (-0.5,-0.5)node [pos=0.9] (lefttop){};

      \foreach \pos in {0.8,0.7,...,0}
      {
      \path (0,1) -- (0,-0.8) node [pos=\pos] (middlebot){};
      \path (0.5,1.3) -- (0.5,-0.5) node [pos=\pos] (rightbot){};
      \path (-0.5,1.3) -- (-0.5,-0.5)node [pos=\pos] (leftbot){};

%
%      \draw (righttop.center)-- (middletop.center) -- (lefttop.center);
%
%      \draw (rightmid.center)-- (middlemid.center) -- (leftmid.center);
		\draw[line width=0.2] (rightbot.center)-- (middlebot.center) -- (leftbot.center);
   }
    \foreach \pos in {0.75,0.5,...,0}
    {
		\draw (0.5,1.3) -- (0,1) node [pos=\pos] (w1-1){};
      \path (0.5,1.3) -- (0,1) node [pos=\pos]{};
      \draw (0.5,-0.5)--(0,-0.8) node [pos=\pos](w1-2){};

      \draw[line width=0.1] (w1-1.center) -- (w1-2.center);
    }
      \draw (-0.5,1.3) -- (0,1);
		\draw (-0.5,-0.5) -- (0,-0.8);
     \foreach \pos in {0.75,0.5,...,0}
    {
		\path (-0.5,1.3) -- (0,1)node [pos=\pos](x1){};
		\path (-0.5,-0.5) -- (0,-0.8) node [pos=\pos](x2){};
      \draw[line width=0.1] (x1.center)--(x2.center);
     }
      \draw (0.5,-0.5)--(0,-0.8) node [pos=0.75](w1-2){};
      \draw (0,1.6) -- (-0.5,1.3) node [pos=0.75]{};
      \draw (0,1.6) -- (0.5,1.3) node [pos=0.75]{};


%		\path (0,1) -- (0,-0.8) node [pos=0.6]  (middletop){};
%		\path (0,1) -- (0,-0.8) node [pos=0.9] (middlebot){};
%      \path (0,1) -- (0,-0.8) node [pos=0.45] (middlemid){};
%		\path (0.5,1.3) -- (0.5,-0.5) node [pos=0.7] (righttop){};
%      \path (0.5,1.3) -- (0.5,-0.5) node [pos=0.9] (rightbot){};
%      \path (0.5,1.3) -- (0.5,-0.5) node [pos=0.45] (rightmid){};
%      \path (-0.5,1.3) -- (-0.5,-0.5)node [pos=0.6] (lefttop){};
%		\path (-0.5,1.3) -- (-0.5,-0.5)node [pos=0.9] (leftbot){};
%      \path (-0.5,1.3) -- (-0.5,-0.5)node [pos=0.45] (leftmid){};
%
%		\draw (righttop.center)-- (middletop.center) -- (lefttop.center);
%%      \draw (rightmid.center)-- (middlemid.center) -- (leftmid.center);
%		\draw (rightbot.center)-- (middlebot.center) -- (leftbot.center);

	}
      \path (-0.5,-0.5) -- (0,-0.8) node [pos=0.5](door1){};
      \node[yslant=-0.6,rectangle,draw] at ($(door1)+(0,0.075)$){};
      \node[yslant=-0.6,circle,draw,scale=0.1,line width=0.2] at ($(door1)+(0.02,0.055)$){};
      \node[yslant=-0.6,circle,draw,scale=0.1,line width=0.2] at ($(door1)+(-0.02,0.075)$){};
	\end{tikzpicture}	
}

\newcommand{\skewedIRS}{
	\begin{tikzpicture}
		\node[rectangle,minimum width=1.5cm,minimum height=1.5cm,draw,yslant=-0.6,scale=0.5,fill=blue!20!green] at (0,0){};

		\node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,yslant=-0.6,scale=0.25,fill=yellow!70!green] (base) at (-0.3,-0.12){};

         \foreach \y in {1,...,5}
         {
            \node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,yslant=-0.6,scale=0.25,fill=yellow!70!green] at
            ($($(base)+(-31:0.14*0)$)+(90:0.12*\y)$){};
         }

      \foreach \x in {1,...,5}
      {
         \node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,yslant=-0.6,scale=0.25,fill=yellow!70!green] at
         ($(base)+(-31:0.14*\x)$){};

         \foreach \y in {1,...,5}
         {
            \node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,yslant=-0.6,scale=0.25,fill=yellow!70!green] at
            ($($(base)+(-31:0.14*\x)$)+(90:0.12*\y)$){};
         }
      }
	\end{tikzpicture}	
}

\newcommand{\IRS}{
	\begin{tikzpicture}
		\node[rectangle,minimum width=1.5cm,minimum height=1.5cm,draw,scale=0.5,fill=blue!20!green] at (0,0){};

		\node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,scale=0.25,fill=yellow!70!green] (base) at (-0.3,-0.3){};

         \foreach \y in {1,...,5}
         {
            \node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,scale=0.25,fill=yellow!70!green] at
            ($($(base)+(-31:0.14*0)$)+(90:0.12*\y)$){};
         }

      \foreach \x in {1,...,5}
      {
         \node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,scale=0.25,fill=yellow!70!green] at
         ($(base)+(0:0.12*\x)$){};

         \foreach \y in {1,...,5}
         {
            \node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,scale=0.25,fill=yellow!70!green] at
            ($($(base)+(0:0.12*\x)$)+(90:0.12*\y)$){};
         }
      }
	\end{tikzpicture}	
}
\tikzset{hexagon/.code={
	\draw (0,2) -- (-4,0) -- (0,-2) -- (4,0) -- (0,2);
}}
\def\phone{{\tikz\node[phone]{};}}
\tikzset{phone/.code={
   \node [rectangle,rounded corners=1.5pt,draw,minimum height=0.6cm, minimum width=0.35cm] at (0,0){};
   \node [rectangle,rounded corners=1.5pt,draw,minimum height=0.5cm, minimum width=0.3cm] at (0,0){};
}}

\newcommand\hcancel[2][black]{\setbox0=\hbox{$#2$}%
\rlap{\raisebox{.45\ht0}{\textcolor{#1}{\rule{\wd0}{1pt}}}}#2}
\makeatletter
% #1, #2 offset of label   #6 extra width to clear arrowhead
% #3, #4 vector direction  #7 superscript label style
% #5 vector width          #8 superscript label
\def\cantox@vector#1#2#3#4#5#6#7#8{%
  \dimen@.5\p@
  \setbox\z@\vbox{\boxmaxdepth.5\p@
   \hbox{\kern-1.2\p@\kern#1\dimen@$#7{#8}\m@th$}}%
  \ifx\canto@fil\hidewidth  \wd\z@\z@ \else \kern-#6\unitlength \fi
  \ooalign{%
    \canto@fil$\m@th \CancelColor
    \vcenter{\hbox{\dimen@#6\unitlength \kern\dimen@
      \multiply\dimen@#4\divide\dimen@#3 \vrule\@depth\dimen@\@width\z@
      \vector(#3,-#4){#5}%
    }}_{\raise-#2\dimen@\copy\z@\kern-\scriptspace}$%
    \canto@fil \cr
    \hfil \box\@tempboxa \kern\wd\z@ \hfil \cr}}
\def\bcancelto#1#2{\let\canto@vector\cantox@vector\cancelto{#1}{#2}}
\makeatother

%\newcommand{\ifthen}[2]{\ifthenelse{#1}{#2}{}}
%\newcommand{\colorRed}[1]{\textcolor{red}{#1}}
%\newcommand{\myNorm}[1]{\left\lVert#1\right\rVert}
%\newcommand{\trNorm}[1]{\left\lVert#1\right\rVert_{\text{Tr}}}
%\newcommand{\tildeV}{\tilde{\vect{v}}}
%\newcommand{\sqr}[1]{{#1}^2}
%\newcommand{\sbrackets}[1]{\left(#1\right)}
%\newcommand{\hbrackets}[1]{\left[#1\right]}
%\newcommand{\vectw}{\vect{\omega}}
%\newcommand{\vectv}{\vect{v}}
%\newcommand{\vectvt}{\tilde{\vect{v}}}
%\newcommand{\matV}{\mat{V}}
%\newcommand{\matX}{\mat{X}}
%\newcommand{\vecth}{\vect{h}}
%\newcommand{\matH}{\mat{H}}
%\newcommand{\vecta}{\vect{a}}
%\newcommand{\matM}{\mat{M}}
%\newcommand{\matOmega}{\mat{W}}
%\newcommand{\vectTheta}{\mat{\theta}}
%\newcommand{\cbrackets}[1]{\left\{#1\right\}}
%\newcommand{\Tr}[1]{\text{Tr}\left(#1\right)}
%\renewcommand{\rank}[1]{\text{rank}\left(#1\right)} 

==> figures/roberts/commands.tex <==
\newcommand{\blank}[1]{\hfil\penalty1000\hfilneg\rule[-3pt]{#1}{0.4pt}} % nice blank underscores
\newcommand{\modernBS}{
	\begin{tikzpicture}[scale=.6]
	{
		\draw (0,1) -- (0,-0.8) node [pos=0.3]  (middletop){};
		\draw (0,1) -- (0,-0.8) node [pos=0.75] (middlebot){};
		\draw (0,1) -- (0.5,-0.5) node [pos=0.3] (righttop){};
		\draw (0,1) -- (0.5,-0.5) node [pos=0.75](rightbot){};
		\draw (0,1) -- (-0.5,-0.5)node [pos=0.3] (lefttop){};
		\draw (0,1) -- (-0.5,-0.5)node [pos=0.75](leftbot){};
		\draw (-0.5,-0.5) -- (0,-0.8) -- (0.5,-0.5);
		\draw (righttop.center)-- (middletop.center) -- (lefttop.center);
		\draw (rightbot.center)-- (middlebot.center) -- (leftbot.center);
	}
	\end{tikzpicture}	
}

% ROBERT
\newcommand{\iPhone}[3]{
	\coordinate (a) at (#1,#2);
	% iPhone case
	\draw [line width=0.25pt,rounded corners=(#3)*1mm,fill=white,scale=(#3)] (a)--($(a)+(0.67,0)$)--($(a)+(0.67,1.381)$)--($(a)+(0,1.381)$)--cycle;
	\draw [color=gray,line width=0.25pt,rounded corners=(#3)*0.8mm,fill=white,scale=(#3)] ($(a)+(0.015,0.015)$)--($(a)+(0.655,0.015)$)--($(a)+(0.655,1.366)$)--($(a)+(0.015,1.366)$)--cycle;
	% Speaker
	\draw [line width=0.25pt,rounded corners=(#3)*0.04mm,scale=(#3)] ($(a)+(0.2875,1.266)$)--($(a)+(0.3825,1.266)$)--($(a)+(0.3825,1.281)$)--($(a)+(0.2875,1.281)$)--cycle;
	% Home button
	\draw[line width=0.25pt,scale=#3] ($(a)+(0.335,0.09)$) circle (0.055cm);
	\draw[line width=0.25pt,scale=#3] ($(a)+(0.335,0.09)$) circle (0.044cm);
	% Front camera
	\draw[line width=0.25pt,scale=#3] ($(a)+(0.2275,1.2735)$) circle (0.015cm);
	% Light sensor
	\draw[line width=0.25pt,scale=#3] ($(a)+(0.335,1.32)$) circle (0.01cm);
	% Display
	\draw [fill={rgb:black,1;white,4},line width=0.25pt,scale=(#3)] ($(a)+(0.042475,0.170195)$)--($(a)+(0.042475,0.170195)+(0.58505,0.0)$)--($(a)+(0.042475,0.170195)+(0.58505,1.04061)$)--($(a)+(0.042475,0.170195)+(0.0,1.04061)$)--cycle;
}
\newcommand{\basestationfiveant}[3]{
	% Macro-cell Basestation
	\coordinate (a) at (#1,#2);
	\draw[line width=(#3)*1.5pt,scale=#3] ($(a)+(0, -1.08)$) -- ($(a)+(0, 1)$);
	\draw[line width=(#3)*1.5pt,scale=#3] ($(a)+(0,1)$) .. controls ($(a)+(-0.25,-0.5)$) .. ($(a)+(-0.5,-0.9)$);
	\draw[line width=(#3)*1.5pt,scale=#3] ($(a)+(0,1)$) .. controls ($(a)+(0.25,-0.5)$) .. ($(a)+(0.5,-0.9)$);
	% Gitter No. 1
	\draw[line width=(#3)*1.5pt,scale=#3] ($(a)+(0, -0.9)$) -- ($(a)+(-0.35, -0.7)$);
	\draw[line width=(#3)*1.5pt,scale=#3] ($(a)+(0, -0.9)$) -- ($(a)+(0.35, -0.7)$);
	\draw[line width=(#3)*0.75pt,scale=#3] ($(a)+(-0.35, -0.65)$) -- ($(a)+(0, -0.5)$);
	\draw[line width=(#3)*0.75pt,scale=#3] ($(a)+(0.35, -0.65)$) -- ($(a)+(0, -0.5)$);
	% Gitter No. 2
	\draw[line width=(#3)*1pt,scale=#3] ($(a)+(0, -0.6)$) -- ($(a)+(-0.3, -0.45)$);
	\draw[line width=(#3)*1pt,scale=#3] ($(a)+(0, -0.6)$) -- ($(a)+(0.3, -0.45)$);
	\draw[line width=(#3)*0.5pt,scale=#3] ($(a)+(-0.3, -0.45)$) -- ($(a)+(0, -0.32)$);
	\draw[line width=(#3)*0.5pt,scale=#3] ($(a)+(0.3, -0.45)$) -- ($(a)+(0, -0.32)$);
	% Gitter No. 3
	\draw[line width=(#3)*0.75pt,scale=#3] ($(a)+(0, -0.3)$) -- ($(a)+(-0.22, -0.17)$);
	\draw[line width=(#3)*0.75pt,scale=#3] ($(a)+(0, -0.3)$) -- ($(a)+(0.22, -0.17)$);
	\draw[line width=(#3)*0.5pt,scale=#3] ($(a)+(-0.22, -0.17)$) -- ($(a)+(0, -0.07)$);
	\draw[line width=(#3)*0.5pt,scale=#3] ($(a)+(0.22, -0.17)$) -- ($(a)+(0, -0.07)$);;
	% Gitter No. 4
	\draw[line width=(#3)*0.75pt,scale=#3] (a) -- ($(a)+(-0.18, 0.11)$);
	\draw[line width=(#3)*0.75pt,scale=#3] (a) -- ($(a)+(0.18, 0.11)$);
	\draw[line width=(#3)*0.5pt,scale=#3] ($(a)+(-0.18, 0.11)$) -- ($(a)+(0,0.2)$);
	\draw[line width=(#3)*0.5pt,scale=#3] ($(a)+(0.18, 0.11)$) -- ($(a)+(0,0.2)$);
	% Gitter No. 5
	\draw[line width=(#3)*0.5pt,scale=#3] ($(a)+(0, 0.3)$) -- ($(a)+(-0.1, 0.37)$);
	\draw[line width=(#3)*0.5pt,scale=#3] ($(a)+(0, 0.3)$) -- ($(a)+(0.1, 0.37)$);
	\draw[line width=(#3)*0.25pt,scale=#3] ($(a)+(-0.1, 0.37)$) -- ($(a)+(0, 0.43)$);
	\draw[line width=(#3)*0.25pt,scale=#3] ($(a)+(0.1, 0.37)$) -- ($(a)+(0, 0.43)$);
	% Antenna
	\draw[line width=(#3)*0.75pt,scale=#3] ($(a)+(0, 1.2)$) -- ($(a)+(0,1)$);
	\draw[fill=white,scale=#3] ($(a)+(0, 1.2)$) circle (0.05cm);
	%	 Waves
	%	\draw[line width=(#3)*1pt,decorate,decoration=expanding waves,decoration={segment length=(#3)*10pt},scale=#3] ($(a)+(0, 1.2)$) -- ($(a)+(0, 2.5)$);
	% Antenna Right
	\draw[line width=(#3)*0.75pt,scale=#3] ($(a)+(0.2, 1)$) -- ($(a)+(0,1)$);
	\draw[line width=(#3)*0.75pt,scale=#3] ($(a)+(0.2, 1.2)$) -- ($(a)+(0.2,1)$);
	\draw[fill=white,scale=#3] ($(a)+(0.2, 1.2)$) circle (0.05cm);
	% Antenna Right 2
	\draw[line width=(#3)*0.75pt,scale=#3] ($(a)+(0.4, 1)$) -- ($(a)+(0.2,1)$);
	\draw[line width=(#3)*0.75pt,scale=#3] ($(a)+(0.4, 1.2)$) -- ($(a)+(0.4,1)$);
	\draw[fill=white,scale=#3] ($(a)+(0.4, 1.2)$) circle (0.05cm);
	% Antenna Left
	\draw[line width=(#3)*0.75pt,scale=#3] ($(a)+(-0.2, 1)$) -- ($(a)+(0,1)$);
	\draw[line width=(#3)*0.75pt,scale=#3] ($(a)+(-0.2, 1.2)$) -- ($(a)+(-0.2,1)$);
	\draw[fill=white,scale=#3] ($(a)+(-0.2, 1.2)$) circle (0.05cm);
	% Antenna Left 2
	\draw[line width=(#3)*0.75pt,scale=#3] ($(a)+(-0.4, 1)$) -- ($(a)+(-0.2,1)$);
	\draw[line width=(#3)*0.75pt,scale=#3] ($(a)+(-0.4, 1.2)$) -- ($(a)+(-0.4,1)$);
	\draw[fill=white,scale=#3] ($(a)+(-0.4, 1.2)$) circle (0.05cm);
}
\newcommand{\building}[4]{
	\coordinate (a) at (#1,#2);
	% Right building
	\draw [draw=black,line width=0.35pt,rounded corners=(#3)*1mm,fill=#4!33!white,scale=(#3)] ($(a)+(.9,0)$)--($(a)+(1.8,0)$)--($(a)+(1.8,1.4)$)--($(a)+(.9,1.4)$)--cycle;
	% Right deco
	\draw [draw=black,line width=0.35pt,rounded corners=(#3)*.1mm,fill=yellow,scale=(#3)] ($(a)+(1.2,1)$) rectangle ++(.5,.15);
	\draw [draw=black,line width=0.35pt,rounded corners=(#3)*.1mm,fill=yellow,scale=(#3)] ($(a)+(1.2,.7)$) rectangle ++(.5,.15);
	\draw [draw=black,line width=0.35pt,rounded corners=(#3)*.1mm,fill=yellow,scale=(#3)] ($(a)+(1.2,.4)$) rectangle ++(.5,.15);
	% Main building
	\draw [draw=black,line width=0.35pt,rounded corners=(#3)*1mm,fill=#4!25!white,scale=(#3)] ($(a)+(-.1,0)$)--($(a)+(1.1,0)$)--($(a)+(1.1,2)$)--($(a)+(-.1,2.2)$)--cycle;
	\draw [draw=black,line width=0.35pt,rounded corners=(#3)*.2mm,fill=#4!33!white,scale=(#3)] ($(a)+(-.2,2)$)--($(a)+(1.2,1.8)$)--($(a)+(1.2,2.1)$)--($(a)+(-.2,2.3)$)--cycle;
	% Main deco
	\draw [draw=black,line width=0.35pt,rounded corners=(#3)*.1mm,fill=#4!50!white,scale=(#3)] ($(a)+(.4,0)$) rectangle ++(.4,.6);
	\draw [draw=black,line width=0.35pt,rounded corners=(#3)*.1mm,fill=yellow,scale=(#3)] ($(a)+(.05,.4)$) rectangle ++(.2,.2);
	\draw [draw=black,line width=0.35pt,rounded corners=(#3)*.1mm,fill=yellow,scale=(#3)] ($(a)+(.05,.8)$) rectangle ++(.2,.2);
	\draw [draw=black,line width=0.35pt,rounded corners=(#3)*.1mm,fill=yellow,scale=(#3)] ($(a)+(.05,1.2)$) rectangle ++(.2,.2);
	\draw [draw=black,line width=0.35pt,rounded corners=(#3)*.1mm,fill=yellow,scale=(#3)] ($(a)+(.05,1.6)$) rectangle ++(.2,.2);
	\draw [draw=black,line width=0.35pt,rounded corners=(#3)*.1mm,fill=yellow,scale=(#3)] ($(a)+(.4,.8)$) rectangle ++(.2,.2);
	\draw [draw=black,line width=0.35pt,rounded corners=(#3)*.1mm,fill=yellow,scale=(#3)] ($(a)+(.4,1.2)$) rectangle ++(.2,.2);
	\draw [draw=black,line width=0.35pt,rounded corners=(#3)*.1mm,fill=yellow,scale=(#3)] ($(a)+(.4,1.6)$) rectangle ++(.2,.2);
	\draw [draw=black,line width=0.35pt,rounded corners=(#3)*.1mm,fill=yellow,scale=(#3)] ($(a)+(.75,.8)$) rectangle ++(.2,.2);
	\draw [draw=black,line width=0.35pt,rounded corners=(#3)*.1mm,fill=yellow,scale=(#3)] ($(a)+(.75,1.2)$) rectangle ++(.2,.2);
	\draw [draw=black,line width=0.35pt,rounded corners=(#3)*.1mm,fill=yellow,scale=(#3)] ($(a)+(.75,1.6)$) rectangle ++(.2,.2);
	% Socket
	\draw [draw=black,line width=0.35pt,fill=#4!33!white,scale=(#3)] ($(a)+(-.2,-.05)$)--($(a)+(-.2,.1)$)--($(a)+(1.9,.1)$)--($(a)+(1.9,-.05)$)--cycle;
}
\definecolor{color1}{rgb}{0.0503832136000000,	0.0298028976000000,	0.527974883000000}%
\definecolor{color2}{rgb}{0.493426212287426,	0.0115244183443711,	0.658032128750000}%
\definecolor{color3}{rgb}{0.796382339000000,	0.277979917955297,	0.471322439808427}%
\definecolor{color4}{rgb}{0.972230291500000,	0.581718982058214,	0.254084505027532}%
\definecolor{color5}{rgb}{0.940015097000001,	0.975158357000000,	0.131325517000000}%
\definecolor{color6}{rgb}{0.5258,    0.8335,    0.2881}%
\newcommand{\autonomousdriving}[3]{
	\coordinate (a) at (#1,#2);
	% Little box upper
	\draw [draw=black,line width=.35pt,rounded corners=(#3)*.1mm,fill=black,scale=(#3)] ($(a)+(0.37,0.5)$)--($(a)+(0.53,0.5)$)--($(a)+(0.53,0.78)$)--($(a)+(0.37,0.78)$)--cycle;
	\draw[draw=none,line width=0.25pt,scale=#3,fill=black!10!white] ($(a)+(0.45,0.73)$) circle (0.04cm);
	% Upper body
	\draw [draw=black,line width=2pt,rounded corners=(#3)*1mm,fill=black!10!white,scale=(#3)] ($(a)+(0.125,0.3)$)--($(a)+(0.775,0.3)$)--($(a)+(0.72,0.65)$)--($(a)+(0.18,0.65)$)--cycle;
	% Wheels
	\draw [draw=black,line width=.35pt,rounded corners=(#3)*.4mm,fill=black,scale=(#3)] ($(a)+(0.05,0.1)$)--($(a)+(0.175,0.1)$)--($(a)+(0.175,-0.15)$)--($(a)+(0.05,-0.15)$)--cycle;
	\draw [draw=black,line width=.35pt,rounded corners=(#3)*.4mm,fill=black,scale=(#3)] ($(a)+(0.85,0.1)$)--($(a)+(0.725,0.1)$)--($(a)+(0.725,-0.15)$)--($(a)+(0.85,-0.15)$)--cycle;
	% Steering wheel
	%\draw[draw=black,line width=0.8pt,scale=#3] ($(a)+(0.55,0.4)$) circle (0.1cm);
	% Main body
	\draw [draw=black,line width=0.35pt,rounded corners=(#3)*1.2mm,fill=black,scale=(#3)] ($(a)+(-0.025,0)$)--($(a)+(0.925,0)$)--($(a)+(0.85,0.4)$)--($(a)+(0.05,0.4)$)--cycle;
	% Headlight
	\draw[draw=none,line width=0.25pt,scale=#3,fill=black!10!white] ($(a)+(0.15,0.2)$) circle (0.08cm);
	\draw[draw=none,line width=0.25pt,scale=#3,fill=black!10!white] ($(a)+(0.75,0.2)$) circle (0.08cm);
	% Cooler grill
	\draw [draw=black!10!white,fill=black!10!white,line width=0.2pt,rounded corners=(#3)*.15mm,scale=(#3)] ($(a)+(0.3,0.12)$)--($(a)+(0.6,0.12)$)--($(a)+(0.6,0.08)$)--($(a)+(0.3,0.08)$)--cycle;
}
%%

\newcommand{\modernBSHalo}{
	\begin{tikzpicture}[scale=.6]
	{
		\draw (0,1) -- (0,-0.8) node [pos=0.3]  (middletop){};
		\draw (0,1) -- (0,-0.8) node [pos=0.75] (middlebot){};
		\draw (0,1) -- (0.5,-0.5) node [pos=0.3] (righttop){};
		\draw (0,1) -- (0.5,-0.5) node [pos=0.75](rightbot){};
		\draw (0,1) -- (-0.5,-0.5)node [pos=0.3] (lefttop){};
		\draw (0,1) -- (-0.5,-0.5)node [pos=0.75](leftbot){};
		\draw (-0.5,-0.5) -- (0,-0.8) -- (0.5,-0.5);
		\draw (righttop.center)-- (middletop.center) -- (lefttop.center);
		\draw (rightbot.center)-- (middlebot.center) -- (leftbot.center);

      \draw[yshift=1cm] (0,0.1) ++(-10:.1) arc (10:180-10:.1);
      \draw[yshift=1cm] (0,0.2) ++(-10:.3) arc (10:180-10:.3);
	}
	\end{tikzpicture}	
}

\newcommand{\modernBuildingWindow}{
   \begin{tikzpicture}
%      \node[rectangle,draw,minimum width=] at (0,0){};
   \end{tikzpicture}
}

\newcommand{\modernBuilding}{
	\begin{tikzpicture}[scale=2]
	{
		\draw (0,1) -- (0,-0.8) node [pos=0.9]  (middletop){};
		\draw (0.5,1.3) -- (0.5,-0.5) node [pos=0.9] (righttop){};
      \draw (-0.5,1.3) -- (-0.5,-0.5)node [pos=0.9] (lefttop){};

      \foreach \pos in {0.8,0.7,...,0}
      {
      \path (0,1) -- (0,-0.8) node [pos=\pos] (middlebot){};
      \path (0.5,1.3) -- (0.5,-0.5) node [pos=\pos] (rightbot){};
      \path (-0.5,1.3) -- (-0.5,-0.5)node [pos=\pos] (leftbot){};

%
%      \draw (righttop.center)-- (middletop.center) -- (lefttop.center);
%
%      \draw (rightmid.center)-- (middlemid.center) -- (leftmid.center);
		\draw[line width=0.2] (rightbot.center)-- (middlebot.center) -- (leftbot.center);
   }
    \foreach \pos in {0.75,0.5,...,0}
    {
		\draw (0.5,1.3) -- (0,1) node [pos=\pos] (w1-1){};
      \path (0.5,1.3) -- (0,1) node [pos=\pos]{};
      \draw (0.5,-0.5)--(0,-0.8) node [pos=\pos](w1-2){};

      \draw[line width=0.1] (w1-1.center) -- (w1-2.center);
    }
      \draw (-0.5,1.3) -- (0,1);
		\draw (-0.5,-0.5) -- (0,-0.8);
     \foreach \pos in {0.75,0.5,...,0}
    {
		\path (-0.5,1.3) -- (0,1)node [pos=\pos](x1){};
		\path (-0.5,-0.5) -- (0,-0.8) node [pos=\pos](x2){};
      \draw[line width=0.1] (x1.center)--(x2.center);
     }
      \draw (0.5,-0.5)--(0,-0.8) node [pos=0.75](w1-2){};
      \draw (0,1.6) -- (-0.5,1.3) node [pos=0.75]{};
      \draw (0,1.6) -- (0.5,1.3) node [pos=0.75]{};


%		\path (0,1) -- (0,-0.8) node [pos=0.6]  (middletop){};
%		\path (0,1) -- (0,-0.8) node [pos=0.9] (middlebot){};
%      \path (0,1) -- (0,-0.8) node [pos=0.45] (middlemid){};
%		\path (0.5,1.3) -- (0.5,-0.5) node [pos=0.7] (righttop){};
%      \path (0.5,1.3) -- (0.5,-0.5) node [pos=0.9] (rightbot){};
%      \path (0.5,1.3) -- (0.5,-0.5) node [pos=0.45] (rightmid){};
%      \path (-0.5,1.3) -- (-0.5,-0.5)node [pos=0.6] (lefttop){};
%		\path (-0.5,1.3) -- (-0.5,-0.5)node [pos=0.9] (leftbot){};
%      \path (-0.5,1.3) -- (-0.5,-0.5)node [pos=0.45] (leftmid){};
%
%		\draw (righttop.center)-- (middletop.center) -- (lefttop.center);
%%      \draw (rightmid.center)-- (middlemid.center) -- (leftmid.center);
%		\draw (rightbot.center)-- (middlebot.center) -- (leftbot.center);

	}
      \path (-0.5,-0.5) -- (0,-0.8) node [pos=0.5](door1){};
      \node[yslant=-0.6,rectangle,draw] at ($(door1)+(0,0.075)$){};
      \node[yslant=-0.6,circle,draw,scale=0.1,line width=0.2] at ($(door1)+(0.02,0.055)$){};
      \node[yslant=-0.6,circle,draw,scale=0.1,line width=0.2] at ($(door1)+(-0.02,0.075)$){};
	\end{tikzpicture}	
}

\newcommand{\skewedIRS}{
	\begin{tikzpicture}
		\node[rectangle,minimum width=1.5cm,minimum height=1.5cm,draw,yslant=-0.6,scale=0.5,fill=blue!20!green] at (0,0){};

		\node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,yslant=-0.6,scale=0.25,fill=yellow!70!green] (base) at (-0.3,-0.12){};

         \foreach \y in {1,...,5}
         {
            \node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,yslant=-0.6,scale=0.25,fill=yellow!70!green] at
            ($($(base)+(-31:0.14*0)$)+(90:0.12*\y)$){};
         }

      \foreach \x in {1,...,5}
      {
         \node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,yslant=-0.6,scale=0.25,fill=yellow!70!green] at
         ($(base)+(-31:0.14*\x)$){};

         \foreach \y in {1,...,5}
         {
            \node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,yslant=-0.6,scale=0.25,fill=yellow!70!green] at
            ($($(base)+(-31:0.14*\x)$)+(90:0.12*\y)$){};
         }
      }
	\end{tikzpicture}	
}

\newcommand{\IRS}{
	\begin{tikzpicture}
		\node[rectangle,minimum width=1.5cm,minimum height=1.5cm,draw,scale=0.5,fill=blue!20!green] at (0,0){};

		\node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,scale=0.25,fill=yellow!70!green] (base) at (-0.3,-0.3){};

         \foreach \y in {1,...,5}
         {
            \node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,scale=0.25,fill=yellow!70!green] at
            ($($(base)+(-31:0.14*0)$)+(90:0.12*\y)$){};
         }

      \foreach \x in {1,...,5}
      {
         \node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,scale=0.25,fill=yellow!70!green] at
         ($(base)+(0:0.12*\x)$){};

         \foreach \y in {1,...,5}
         {
            \node[rectangle,minimum width=0.05cm,minimum height=0.05cm,draw,scale=0.25,fill=yellow!70!green] at
            ($($(base)+(0:0.12*\x)$)+(90:0.12*\y)$){};
         }
      }
	\end{tikzpicture}	
}
\tikzset{hexagon/.code={
	\draw (0,2) -- (-4,0) -- (0,-2) -- (4,0) -- (0,2);
}}
\def\phone{{\tikz\node[phone]{};}}
\tikzset{phone/.code={
   \node [rectangle,rounded corners=1.5pt,draw,minimum height=0.6cm, minimum width=0.35cm] at (0,0){};
   \node [rectangle,rounded corners=1.5pt,draw,minimum height=0.5cm, minimum width=0.3cm] at (0,0){};
}}

\newcommand\hcancel[2][black]{\setbox0=\hbox{$#2$}%
\rlap{\raisebox{.45\ht0}{\textcolor{#1}{\rule{\wd0}{1pt}}}}#2}
\makeatletter
% #1, #2 offset of label   #6 extra width to clear arrowhead
% #3, #4 vector direction  #7 superscript label style
% #5 vector width          #8 superscript label
\def\cantox@vector#1#2#3#4#5#6#7#8{%
  \dimen@.5\p@
  \setbox\z@\vbox{\boxmaxdepth.5\p@
   \hbox{\kern-1.2\p@\kern#1\dimen@$#7{#8}\m@th$}}%
  \ifx\canto@fil\hidewidth  \wd\z@\z@ \else \kern-#6\unitlength \fi
  \ooalign{%
    \canto@fil$\m@th \CancelColor
    \vcenter{\hbox{\dimen@#6\unitlength \kern\dimen@
      \multiply\dimen@#4\divide\dimen@#3 \vrule\@depth\dimen@\@width\z@
      \vector(#3,-#4){#5}%
    }}_{\raise-#2\dimen@\copy\z@\kern-\scriptspace}$%
    \canto@fil \cr
    \hfil \box\@tempboxa \kern\wd\z@ \hfil \cr}}
\def\bcancelto#1#2{\let\canto@vector\cantox@vector\cancelto{#1}{#2}}
\makeatother

%\newcommand{\ifthen}[2]{\ifthenelse{#1}{#2}{}}
%\newcommand{\colorRed}[1]{\textcolor{red}{#1}}
%\newcommand{\myNorm}[1]{\left\lVert#1\right\rVert}
%\newcommand{\trNorm}[1]{\left\lVert#1\right\rVert_{\text{Tr}}}
%\newcommand{\tildeV}{\tilde{\vect{v}}}
%\newcommand{\sqr}[1]{{#1}^2}
%\newcommand{\sbrackets}[1]{\left(#1\right)}
%\newcommand{\hbrackets}[1]{\left[#1\right]}
%\newcommand{\vectw}{\vect{\omega}}
%\newcommand{\vectv}{\vect{v}}
%\newcommand{\vectvt}{\tilde{\vect{v}}}
%\newcommand{\matV}{\mat{V}}
%\newcommand{\matX}{\mat{X}}
%\newcommand{\vecth}{\vect{h}}
%\newcommand{\matH}{\mat{H}}
%\newcommand{\vecta}{\vect{a}}
%\newcommand{\matM}{\mat{M}}
%\newcommand{\matOmega}{\mat{W}}
%\newcommand{\vectTheta}{\mat{\theta}}
%\newcommand{\cbrackets}[1]{\left\{#1\right\}}
%\newcommand{\Tr}[1]{\text{Tr}\left(#1\right)}
%\renewcommand{\rank}[1]{\text{rank}\left(#1\right)} 

==> sections/transmission_scheme.tex <==
\section{Transmission Scheme}

